MIGRO: A Decoupled and Portable Long-Term Memory System for Language Models

Language models evolve, but the observations, revisions, and context accumulated through user interactions should remain usable. Each new model must be able to retrieve past evidence, track revisions, and add new observations. We present MIGRO, a decoupled long-term memory system that treats experience as a persistent state shared across successive language models. MIGRO follows a simple principle: preserve historical evidence exactly, organize it approximately, and decide what to retrieve only when the question is known. We call this asymmetric fidelity with deferred selectivity. A shared semantic index supports retrieval, while exact records retain observations and their historical relationships. Because models differ in vocabulary and tokenization, host-specific interfaces convert selected evidence into inputs the receiving model can use. Reversible encoding reduces archival storage while enabling exact recovery. The shared state and its access interfaces let successive hosts read and extend the accumulated experience. On matched LoCoMo states, MIGRO scores 7.3% higher and uses 99.3% less private memory than the strongest quality baseline. After handoff, continued writing retains 99.9% of full-history rebuilding quality by extending the inherited state. On million-token BEAM histories, MIGRO uses 57.5% less private storage on average than the most compact baseline. MIGRO combines high answer quality, continued memory growth across hosts, and low storage cost. Code is available at https://github.com/zOUMINGXI/MIGRO.

==> sections/storage_additional.tex <==
\FloatBarrier
\section{Additional LoCoMo Storage Results}
\label{sec:storageadditional}
The ten matched conversations provide a shorter-history view of continued writing. At each prefix, Figure~\ref{fig:locomogrowth} compares the same eligible conversations; their count decreases with length. Figure~\ref{fig:locomomarginal} measures byte increments within each conversation before averaging. MIGRO's second-half cost is 4.207 bytes/token, versus 8.847 for LSTMem, 49.385 for TiMem, 113.668 for A-MEM, 410.676 for PlugMem, and 820.634 for Mem0. These measurements complement the matched-state quality comparison in Section~\ref{sec:storage}.

\begin{figure}[H]
\centering
\includegraphics[width=.87\linewidth]{figures/storage_conversation_storage_growth.pdf}
\caption{LoCoMo native memory growth across the same eligible conversations at each prefix. Counts above the plot show the available natural histories.}
\label{fig:locomogrowth}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=.87\linewidth]{figures/storage_late_marginal_storage.pdf}
\caption{LoCoMo incremental storage. Left: later-history windows. Right: mean second-half cost and 95\% conversation-bootstrap intervals; MIGRO averages 4.207 bytes/token.}
\label{fig:locomomarginal}
\end{figure}
\FloatBarrier

